BrazilDAM: A Benchmark dataset for Tailings Dam Detection

In this work we present BrazilDAM, a novel public dataset based on Sentinel-2 and Landsat-8 satellite images covering all tailings dams cataloged by the Brazilian National Mining Agency (ANM). The dataset was built using georeferenced images from 769 dams, recorded between 2016 and 2019. The time series were processed in order to produce cloud free images. The dams contain mining waste from different ore categories and have highly varying shapes, areas and volumes, making BrazilDAM particularly interesting and challenging to be used in machine learning benchmarks. The original catalog contains, besides the dam coordinates, information about: the main ore, constructive method, risk category, and associated potential damage. To evaluate BrazilDAM's predictive potential we performed classification essays using state-of-the-art deep Convolutional Neural Network (CNNs). In the experiments, we achieved an average classification accuracy of 94.11% in tailing dam binary classification task. In addition, others four setups of experiments were made using the complementary information from the original catalog, exhaustively exploiting the capacity of the proposed dataset.

==> tex/applications.tex <==



\section{Applications}

Access to data allows for a variety of approaches, both in real-life  applications and other types of research. Some of the applications such as detection and label classification were even the motivations of this work. But the dataset has a lot of additional information that can still be explored, and that's what we'll talk about in this session.

% \subsection{Unregistered dam detection}

% According to ANA (Agência Nacional de Águas), Brazilian National Water Agency, a large part of the ore dams have not yet been registered or cataloged in the national safety policy. This is expensive work and requires a lot of manpower to cover the entire Brazilian territory.
% %https://www.ana.gov.br/noticias/45-barragens-preocupam-orgaos-fiscalizadores-aponta-relatorio-de-seguranca-de-barragens-elaborado-pela-ana

% While there is a duty for companies to report dam construction, they often do not, causing soil contamination or disruption due to poor planning.
% Using the detection algorithm shown in this article, it is possible to make these records remotely and much faster with 92\% accuracy in the worst case. 

% \subsection{Classification in ore type, construtive method, risk category and associeted potencial damage.}

% Using the same argument as detecting unregistered dams, the cost to label any dam on a dam is high, with a large staff and takes a long time. Therefore, with the application of remote sensing CNNs, this manual work becomes automatic, with a small rate of errors compared or even smaller than human errors.

% The classification of the type of ore that is extracted and its tailings are stored in the dams, is a complex work due to the construction proportions. The dam is like a barrier, where the tailings generated in the ore beneficiation process are disposed in a controlled, planned and insured manner. However, when different types of unplanned tailings are added, due to the density and decantation of some elements, unwanted pressure is created at the base of the structure which can lead to cracking and eventual breakage.

% Inspection of the construction method is another approach that can be viewed in terms of monitoring whether all constructions are being made in accordance with previously established requirements. There is a difference in costs between these types, as there is also a difference in security level, the upstream method is cheaper than the juxtaposed method by examples, but the latter is safer.

% The categorization of risk and associated potential damage has direct influence, disasters such as those in Brazil could have been prevented by large-scale oversight and preparation of nearby regions where the potential for risk is high.
% Knowing this data quickly and easily enables responsible agents to focus on ways to prevent and, in the worst cases, build more robust security protocols.

\subsection{Super Resolution}

The proposed dataset has a multispectral and multisensor approach, with two satellites with slight differences, one of which is the resolution of the bands. Visible bands have 10 meters per pixel in Sentinel and 30 meters per pixel in Landsat, this allows super-resolution methods to be applied to try to improve classifications with low-resolution images like Landsat's, and validate in Sentinel images, making the dataset very rich for this application, An example of this kind of difference can be seen in Figure \ref{fig:superresolution}.

Although Sentinel has good resolution images, it was released in 2015 while Landsat8 was released in 2013, and with this application, you can get a lot of older images with better resolution.

\begin{figure}[h]
\subfigure[Landsat Image]{
    \includegraphics[width=.475\columnwidth]{images/001_landsat.png}
    %\label{fig:subfig1}
}
\subfigure[Sentinel Image]{
    \includegraphics[width=.475\columnwidth]{images/001_sentinel.png}
    %\label{fig:subfig2}
}

%Exemplos de barragens de diferentes métodos de construção dentro da mesma regiao. Na imagem (a), apresenta uma barragem construida usando o método de Alteamento a Montante, enquanto em uma região proxima, temos a imagem (b) de uma barragem construida usando o método de etapa única

\caption[]{Examples of images from the same region of different satellites.}
\label{fig:superresolution}
\end{figure}

\subsection{Change Detection}

Change detection is an old problem that suffers from the amount of labeled data. The time axis of the dataset can be explored for this purpose, the characteristics of relevant changes can be studied between every year in pairs, making the amount of information highly scalable.

As the dams change due to their use, the application in detecting detection is clear. Also one of the ways to observe the risk of rupture is from the amount of slope movement, the slanted ground plan that limits a landfill and its function is to ensure the stability of the landfill, when there is some movement over time is a warning sign and this alert can be measured quantitatively by how much movement there was, or in this case, change.

\begin{figure}[h]
\subfigure[2016 image]{
    \includegraphics[width=.475\columnwidth]{images/159_2016.png}
    %\label{fig:subfig1}
}
\subfigure[2019 image]{
    \includegraphics[width=.475\columnwidth]{images/159_2019.png}
    %\label{fig:subfig2}
}

%Exemplos de barragens de diferentes métodos de construção dentro da mesma regiao. Na imagem (a), apresenta uma barragem construida usando o método de Alteamento a Montante, enquanto em uma região proxima, temos a imagem (b) de uma barragem construida usando o método de etapa única

\caption[]{Examples of images from the same region in different times.}
\label{fig:changedetection}
\end{figure}

%\ede{Discussão sobre possiveis formas de explorar o dataset proposto: Super Resolução, Change Detection, ???, ???}



==> tex/related_work.tex <==
\section{Related Work}

%In this section we present some of the available datasets in the literature about the remote sensing classification task.  In the following, the methods considered state-of-the-art in classification tasks are shown.

One of the first widely used remote sensing and image classification datasets was proposed in \cite{yang2010bag}, and used in high relevance publications as \cite{penatti2015deep,hu2015transferring,cheng2016survey}. The dataset covers a total of 21 agricultural to parking image classes, extracted from images from the USGS National Map Urban Area Imagery collection. Overall, the dataset contains 100 images per class in visible spectrum (totaling 2100 RGB images), 256x256 pixels and a spatial resolution of 0.30m. Exploring Near Infrared (NIR) information, the authors in \cite{basu2015deepsat} proposed the SAT-4 and SAT-6 datasets. Both datasets have 500,000 patches of 28x28 size images with 4 bands RGB-NIR with spatial resolution of 0.30m. All images were taken from National Agriculture Imagery Program (NAIP) 2009.

%The authors in \cite{cheng2017remote} proposed RESISC45 by using a wide range of scenes. 
The dataset RESISC45~\cite{cheng2017remote} uses 31,500 images divided into 45 different classes covering regions from around the world. Each class is represented by 700 256x256 size images in the visible (RGB) spectrum, varying the spatial resolution from 30m to 0.2m per pixel. The acquisition of the images was done through the Google Earth tool, and its labels through remote sensing professionals. 


% Cortado para camera ready
% In the competition environment, datasets such as Kaggle-planet, Statoil / C-CORE Iceberg and Cactus Aerial Photos were created and explored. In the Kaggle planet dataset, 256x256 images with 5m spatial resolution are available in the RGB-NIR of the Amazon basin region. In this case, the classification task is divided into 13 land cover categories plus 4 cloud condition categories and aims to track the human footprint in the Amazon rainforest and better understand the deforestation phenomenon. Using elevation images, in the Statoil / C-CORE Iceberg dataset it is proposed to identify drifting icebergs in navigational and coastal areas. For this purpose, 75x75 images are available using the 2-band HH / HV SAR sensor, divided between the ship or iceberg classes. Using unmanned aerial vehicle, \cite{lopez2019columnar} proposed the Cactus Aerial Photos dataset for monitoring biodiversity endemic plants. The dataset is composed of 17k RGB images of size 32x32 aerial from the categories cactus and non-cactus. Using sentinel satellite 2 for image acquisition, as well as this work, the BigEarthNet, EuroSAT, LCZ42 datasets were proposed by  \cite{sumbul2019bigearthnet}, \cite{helber2019eurosat}, \cite{zhu2019so2sat}, respectively. 


Despite the number of publications with experimental evaluations on new datasets, often when the data is of high quality, the data is not freely available to the public. In addition, much of the research focused on specific remote sensing applications is sponsored by private companies, which end up acquiring non-free high resolution spatial or spectral images in regions of interest of the application.

Computational techniques involving machine learning and statistical learning have been used with great success in several applications in the context of computer vision, including remote sensing. Advances in computer vision tasks have long been limited due to the effectiveness of handcraft feature-based image description algorithms. However with the resurgence of deep neural networks and especially the so-called Convolutional Neural Networks (CNNs) this scenario has changed. Convolutional neural networks are capable of extracting highly descriptive feature vectors, since it has a natural ability to effectively encode spectral and spatial information based mainly on the data itself. Methods based on deep learning have obtained state-of-the-art results in many different Earth Observation applications, such as image classification \cite{penatti2015deep}, semantic segmentation \cite{volpi2016dense}, phenological studies \cite{nogueira2019spatio}, etc. In this paper, we select six networks architectures considered as state of the art (\cite{krizhevsky2014one}, \cite{huang2017densely}, \cite{szegedy2016rethinking}, \cite{he2016deep}, \cite{iandola2016squeezenet}, \cite{simonyan2014very}) and evaluate the proposed dataset predictive potential.



%The  presented  works  extensively  evaluated  all proposed  machine  learning  methods  and  concluded  that  thatdeep CNNs outperform non-deep learning approaches on theconsidered dataset

%highly descriptive feature extractors like convolutional neural networks, the whole area of image analysis has shown a significant increase in accuracy


%Methods based on deep learning have obtained state-of-the-art results in many di fferent Earth Observation applications, such as image classification [Chen et al., 2014; Firat et al., 2014; Zhang et al., 2015; Guan et al., 2015; Penatti et al., 2015; Lin, 2016], semantic segmentation [Paisitkriangkrai et al., 2015; Nogueira et al., 2015b; Yue et al., 2015; Paisitkriangkrai et al., 2015; Marmanis et al., 2018; Sherrah, 2016; Chen et al., 2016; Volpi and Tuia, 2017; Nogueira et al., 2019a], poverty mapping [Xie et al., 2016], phenological studies [Nogueira et al., 2016b, 2017a, 2019b], and so on.


%Semantic segmentation is an image analysis task that assigns for every pixel in an input image a label that describes the class of its enclosing region. Beyond image classification and object detection, semantic segmentation is the highest-level image analysis task that allows a complete scene understanding of the whole input image.      

%Semantic segmentation was referred in many remote sensing works as pixel-wise classification. Semantic segmentation term is more used in computer vision, and it is being more and more adopted in remote sensing. Semantic segmentation can be used in aerial imagery in a variety of  potential applications, like urban area monitoring and planning, traffic management and analysis, hazard detection and avoidance, and so on. This potential is boosted by the increasing adoption of unmanned aerial vehicles (UAVs). UAVs make the surveillance of inhabited areas easier due to their flexibility, great mobility, and the high resolution images that they can gather and stream in real time. These images can be automatically processed by accurate semantic segmentation algorithms to substantially reinforce the ability to analyze and describe the surveyed scenes automatically.

%The progress of semantic segmentation algorithms was delayed years ago by the low accuracy of traditional approaches of image analysis algorithms based on the extraction of hand-crafted features. However, since the emergence of highly descriptive feature extractors like convolutional neural networks, the whole area of image analysis has shown a significant increase in accuracy. In fact, since 2012 [1], convolutional neural networks (CNNs) have shown an outstanding efficiency in computer vision. This advancement enhanced the areas of semantic segmentation algorithms. Recently, several CNN- based architectures have shown their efficiency in this task, such as fully connected networks (FCN) [2], SegNet [3], UNet [4], PSPNets [5], and DeepLab [6]. If a robust dataset is provided and semantically labeled, training one of the state-of-the-art models could lead easily to an accuracy that exceeds 80% [7].




%To the best of our knowledge, our dataset is the first dataset of Brazil's tailings dams. 

%of the largest scale on the number of scene classes and the total image number. The creation  of  this  new  dataset  will  enable  the  community  to develop and test various data-driven algorithms to further boost the state-of-the-arts.


%lmost all existing datasets are small scale. To address this problem, we propose a large-scale, freely and publicly available benchmark dataset, which covers 31,500 images and 45 scene classes with 700 images per class. Taking the most widely-used UC Merced dataset [38] as comparison, the total image number of our dataset is 15 times larger than it. 


% Falar de uns 3 datasets de barragem



%Compared  to  the  EuroSAT  dataset  presented  in  this  work,the  previously  listed  datasets  rely  on  commercial  very-high-resolution  and  preprocessed  images.  The  fact  of  using  com-mercial   and   preprocessed   very-high-resolution   image   datamakes  these  datasets  unsatisfying  for  real-world  Sentinel-2  Earth  observation  applications  as  proposed  in  this  work.Furthermore,   while   these   datasets   put   a   strong   focus   onstrengthening  the  number  of  covered  classes,  the  datasetssuffer  from  a  low  number  of  images  per  class.  The  fact  of  aspatial resolution of up to 30 cm per pixel, with the possibilityto identify and distinguish classes like churches, schools etc.,make  the  presented  datasets  difficult  to  compare  with  thedataset proposed in this work.A  study  closer  to  our  work,  provided  by  Penatti  et  al.[20], analyzed remotely sensed satellite images with a spatialresolution  of  10  meters  per  pixel  to  classify  coffee  crops.Based  on  these  images,  Penatti  et  al.  [20]  introduced  theBrazillian  Coffee  Scene  (BCS)  dataset.  The  dataset  coversthe  two  classes  coffee  crop  and  non-coffee  crop.  Each  classconsists of 1,423 images. The images consist of a red, greenand near-infrared band.


%https://www.kaggle.com/c/planet-understanding-the-amazon-from-space/overview


%1)  Large  scale: The resurrection of deep learning has had a revolutionary impact on the current state-of-the-arts in machine learning and computer vision. A major contributing factor to its success is the availability of large-scale datasets that allows deep networks to develop their full potential. Unfortunately, as can be seen from Table 1, almost all existing datasets are small scale. To address this problem, we propose a large-scale, freely and publicly available benchmark dataset, which covers 31,500 images and 45 scene classes with 700 images per class. Taking the most widely-used UC Merced dataset [38] as comparison, the total image number of our dataset is 15 times larger than it. 
%To the best of our knowledge, our dataset is of the largest scale on the number of scene classes and the total image number. The creation  of  this  new  dataset  will  enable  the  community  to develop and test various data-driven algorithms to further boost the state-of-the-arts. 

%2) Rich image variations: Tolerance to image variations is an important desired property of any scene classification system, be it human or machine. However, most of the existing datasets are not very rich in terms of image variations. On the contrary, our images were carefully selected under all kinds of weathers, seasons, illumination conditions, imaging conditions, and scales. Thus, for each scene category, our dataset possesses much rich variations in translation, viewpoint, object pose and appearance, spatial resolution, illumination, background, and occlusion, etc.  

%3) High within class diversity and between class similarity:Many top-performing methods built upon deep neural networks have achieved saturation of classification accuracy on most of the existing datasets owing to their simplicity, or rather the lack of variations and diversity. With this in mind, our new dataset is rather challenging with high within class diversity and between class similarity. To this end, we obtained images under all kinds of conditions and added some more fine-grained scene classes with high semantic overlapping such as circular farmland and rectangular  farmland,  commercial  area  and  industrial  area, basketball court and tennis court, and so on. In the 


%Abstract—In  this  paper,  we  address  the  challenge  of  land  useand land cover classification using Sentinel-2 satellite images. TheSentinel-2  satellite  images  are  openly  and  freely  accessible  pro-vided in the Earth observation program Copernicus. We presenta  novel  dataset  based  on  Sentinel-2  satellite  images  covering  13spectral bands and consisting out of 10 classes with in total 27,000labeled  and  geo-referenced  images.  We  provide  benchmarks  forthis  novel  dataset  with  its  spectral  bands  using  state-of-the-artdeep Convolutional Neural Network (CNNs). With the proposednovel  dataset,  we  achieved  an  overall  classification  accuracy  of98.57%. The resulting classification system opens a gate towardsa  number  of  Earth  observation  applications.  We  demonstratehow  this  classification  system  can  be  used  for  detecting  landuse  and  land  cover  changes  and  how  it  can  assist  in  improvinggeographical maps. The geo-referenced dataset EuroSAT is madepublicly  available  at  https://github.com/phelber/eurosat


%Deepsat: SAT-4/SAT-6 airborne datasets (Louisiana State University, 2015) 6 land cover categories, 400k 28x28 pixel chips, 4-band RGBNIR aerial imagery (1m res.) extracted from the 2009 National Agriculture Imagery Program (NAIP), Paper: Basu et al. 2015



%BigEarthNet: Large-Scale Sentinel-2 Benchmark (TU Berlin, Jan 2019)
%Multiple landcover labels per chip based on CORINE Land Cover (CLC) 2018, 590,326 chips from Sentinel-2 L2A scenes (125 Sentinel-2 tiles from 10 European countries, 2017/2018), 66 GB archive, Paper: Sumbul et al. 2019



%So2Sat LCZ42 (TUM Munich & DLR, Aug 2018)
%Local climate zone classification, 17 categories (10 urban e.g. compact high-rise, 7 rural e.g. scattered trees), 400k 32x32 pixel chips covering 42 cities (LCZ42 dataset), Sentinel 1 & Sentinel 2 (both 10m res.), 51 GB


%Functional Map of the World Challenge (IARPA, Dec 2017)
%63 categories from solar farms to shopping malls, 1 million chips, 4/8 band satellite imagery (0.3m res.), COCO data format, baseline models, Paper: Christie et al. 2017

%EuroSAT (DFK, Aug 2017)
%10 land cover categories from industrial to permanent crop, 27k 64x64 pixel chips, 3/16 band Sentinel-2 satellite imagery (10m res.), covering cities in 30 countries, Paper: Helber et al. 2017






%WiDS Datathon 2019 : Detection of Oil Palm Plantations (Global WiDS Team & West Big Data Innovation Hub, Jan 2019) Prediction of presence of oil palm plantations, Planet satellite imagery (3m res.)., ca. 20k 256 x 256 pixel chips, 2 categories oil-palm and other, annotator confidence score.




